SpeechBERT: An Audio-and-text Jointly Learned Language Model for End-to-end Spoken Question Answering

While various end-to-end models for spoken language understanding tasks have been explored recently, this paper is probably the first known attempt to challenge the very difficult task of end-to-end spoken question answering (SQA). Learning from the very successful BERT model for various text processing tasks, here we proposed an audio-and-text jointly learned SpeechBERT model. This model outperformed the conventional approach of cascading ASR with the following text question answering (TQA) model on datasets including ASR errors in answer spans, because the end-to-end model was shown to be able to extract information out of audio data before ASR produced errors. When ensembling the proposed end-to-end model with the cascade architecture, even better performance was achieved. In addition to the potential of end-to-end SQA, the SpeechBERT can also be considered for many other spoken language understanding tasks just as BERT for many text processing tasks.

==> sections/discussion.tex <==

\vspace{-5pt}
\section{Discussions and future works}



\vspace{-5pt}
Though we achieved a reasonable performance on the SQA task, there is still a large room for future research. The first challenge is the usage of word boundaries. Although it is legal to use an off-the-shelf ASR model that acts as a segmenter under a supervised setting, it will be much more desirable if the boundaries can be provided by the end-to-end model itself. In conventional SLU tasks, it is possible to extract information from frame-level speech features to do sentence-level classification tasks like slot filling. However, it will be an enormous challenge to use frame-level speech features for the SQA model which needs a pointer network to predict positions directly on very long frames. In this work, we choose an easier setting that focuses on embedding learning and language model pre-training to solve SQA with pre-computed word boundaries. One possible way to integrate segmentation into our approach is simply dividing audios by the voice intensity. Alternatively, previous work on simultaneous speech translation~\cite{oda2014optimizing} has proposed algorithms to learn segmentation strategies that directly maximizes the performance of the machine translation system. 

Joint learning of segmentation and audio embedding that can mutually be enhanced by reinforcement learning~\cite{wang2018segmental} is another promising approach. This method can be adapted to the text and speech cross-modal language model pre-training in our work in the future.

The second goal for future research is cross-modal langauge model pre-training with few labels for speech corpus. While paired data was used in our pre-training stage, semi-supervised or unsupervised method can leverage the much larger unpaired corpora. 


==> sections/relatedworks.tex <==
\section{Related Works}
\label{sec:relatedworks}

\subsection{Speech Segment Embedding}
\label{ssec:sse}

\vspace{-5pt}
In a series of investigations, people want to extract semantic embeddings from speech feature segments given predefined segment boundaries. Speech2Vec~\cite{speech2vec2018} used a speech feature level sequence-to-sequence network to imitate the training process of skip-gram or CBOW in Word2Vec~\cite{mikolov2013distributed} to help the model extract more semantic feature. Unsupervised segmentation method~\cite{wang2018segmental} was also proposed to jointly learn to segment spoken words and extract the speech embeddings. After learning the speech segment embeddings, the following works~\cite{yichen2018, chung2019nips} tried to map them to a regular word embedding, as we do in bilingual embedding mapping~\cite{conneau2017}, either in supervised (using paired seeds) or unsupervised (using Generative Adversarial Networks~\cite{goodfellow2014generative}) approaches. Promising as these works sound, by now the mapping qualities are far from that of a bilingual embedding mapping case. The correctness of the mapping between speech and text embeddings is at most near 25\% ~\cite{chung2019nips} even with the aid of oracle boundaries. That indicates the difficulty of disentangling semantic information from noisy speech signals without a supervised ASR model.

We also used the speech segment embedding concept in this work. The method will be introduced in \ref{ssec:psje}. However, because the baseline methods of the SQA tasks already include a supervised ASR model as front end, we did not impractically pursue a fully unsupervised method for speech content extraction. Instead, we used the labels of what words are exactly represented by speech segments in the pre-training stage.

\vspace{-3pt}
\subsection{End-to-end Model for Spoken Language Tasks}
\label{ssec:e2e}
\vspace{-5pt}
Conventional methods for spoken language tasks need an ASR as a front-end module to extract semantic information from speech signals into plain text. The output of ASR will be treated as natural language data and fed into regular NLP models for downstream tasks. The end-to-end model aims to tackle the whole task from speech level features without cascading the ASR model. The end-to-end model has the benefits: 1) it optimizes the metric of the final task directly, instead of optimizing toward different targets for ASR and NLP models separately 2) it avoids error propagation problem caused by ASR bottleneck 3) the direct exposure of speech information to downstream models can help the model to capture useful information that is not shown in text transcripts.

Regular spoken language understanding (SLU) tasks like intent classification and slot filling have been explored in end-to-end methods \cite{chen2017reading, haghani2018audio, chen2018spoken, serdyuk2018towards} wider recently compared to spoken question answering (SQA) tasks~\cite{Lee2018spoken}. However, these two tasks are at different levels of difficulty. SLU task is a sentence-level classification problem that needs to fill the slots from pre-defined classes by extracting some local information in a short utterance. As the literal meaning of the short utterance is extracted by the SLU model, it is not far from making a correct classification. Compared to SLU, the inputs in the SQA task are much longer spoken paragraphs. Besides understanding the literal meaning, the SQA model needs to organize the global information first because the sophisticated reasoning in the paragraph is required to answer the questions. Fine-grained information is also needed to predict the exact position of the answer span from a very long context. Therefore, we will solve it by pointer networks\cite{pointernet} instead of classification models. These are the reasons why SQA would be a harder problem than SLU.

